The Demographics of Rocky Free-Floating Planets and their Detectability by WFIRST

Planets are thought to form via accretion from a remnant disk of gas and solids around a newly formed star. During this process material in the disk either remains bound to the star as part of either a planet, a smaller celestial body, or makes up part of the interplanetary medium; falls into the star; or is ejected from the system. Herein we use dynamical models to probe the abundance and properties of ejected material during late-stage planet formation and estimate their contribution to the free-floating planet population. We present 300 N-body simulations of terrestrial planet formation around a solar-type star, with and without giant planets present, using a model that accounts for collisional fragmentation. In simulations with Jupiter and Saturn analogs, about one-third of the initial (~5 Mearth) disk mass is ejected, about half in planets more massive than Mercury but less than 0.3 Mearth, and the remainder in smaller bodies. Most ejections occur within 25 Myr, which is shorter than the timescale typically required for Earth-mass planets to grow (30-100 Myr). When giant planets are omitted from our simulations, almost no material is ejected within 200 Myr and only about 1% of the initial disk is ejected by 2 Gyr. We show that about 2.5 terrestrial-mass planets are ejected per star in the Galaxy. We predict that the space-borne microlensing search for free-floating planets from the Wide-Field Infra-Red Space Telescope (WFIRST) will discover up to 15 Mars-mass planets, but few free-floating Earth-mass planets.

==> macros2.tex <==
\newcommand{\myemail}{elisa.quintana@nasa.gov}





\newcommand{\mearth}{M\ensuremath{_{\oplus}}\xspace} 	
\newcommand{\vkep}{\ensuremath{v_{kep}}\xspace}
\newcommand{\vinf}{\ensuremath{v_{\infty}}\xspace}
\newcommand{\vesc}{\ensuremath{v_{esc}}\xspace}
\newcommand{\venc}{\ensuremath{v_{enc}}\xspace}
\newcommand{\vrel}{\ensuremath{v_{rel}}\xspace}
\newcommand{\timp}{\ensuremath{t_{imp}}\xspace}

\newcommand{\mimp}{\ensuremath{m_{imp}}\xspace}
\newcommand{\mtar}{\ensuremath{m_{tar}}\xspace}
\newcommand{\vimp}{\ensuremath{v_{imp}}\xspace}
\newcommand{\teqstar}{\ensuremath{T_{\mathrm{eq_*}}}\xspace}  
\newcommand{\logg}{\ensuremath{\log g}\xspace}                
\newcommand{\z}{\ensuremath{Z}\xspace} 	
\newcommand{\kepmag}{\ensuremath{K_{\mathrm{p}}}\xspace} 	
\newcommand{\msun}{\ensuremath{M_\odot}\xspace}		          
\newcommand{\mstar}{\ensuremath{M_*}\xspace} 		         
\newcommand{\rsun}{\ensuremath{R_\odot}\xspace} 		          
\newcommand{\rstar}{\ensuremath{R_*}\xspace} 		         
\newcommand{\rhostar}{\ensuremath{\bar{\rho_*}}\xspace} 	
\newcommand{\arstar}{\ensuremath{a/R_*}\xspace} 	
\newcommand{\arstarfrac}{\ensuremath{\frac{a}{R_*}}\xspace} 	
\newcommand{\semimaj}{\ensuremath{\it{a}}\xspace} 	
\newcommand{\semimajC}{\ensuremath{\it{a}}\xspace} 	
\newcommand{\eccC}{\ensuremath{\it{e}}\xspace} 	
\newcommand{\incC}{\ensuremath{\it{i}}\xspace} 	
\newcommand{\lstar}{\ensuremath{L_*}\xspace} 	
\newcommand{\lsun}{\ensuremath{L_\odot}\xspace} 	
% planet parameters
\newcommand{\massp}{\ensuremath{M_{\mathrm{p}}}\xspace} 	
\newcommand{\mjup}{\ensuremath{M_{\mathrm{J}}}\xspace} 	
\newcommand{\mmars}{\ensuremath{M_{\mathrm{Mars}}}\xspace} 	
\newcommand{\mmoon}{\ensuremath{M_{\mathrm{Moon}}}\xspace} 	
\newcommand{\rp}{\ensuremath{r_{\mathrm{p}}}\xspace} 	
\newcommand{\rjup}{\ensuremath{R_{\mathrm{J}}}\xspace} 	
\newcommand{\rearth}{\ensuremath{R_{\oplus}}\xspace} 	
\newcommand{\rhop}{\ensuremath{\bar{\rho_{\mathrm{p}}}}\xspace} 	
\newcommand{\teq}{\ensuremath{T_{\mathrm{eq_p}}}\xspace}  
\newcommand{\teffp}{\ensuremath{T_{\mathrm{eff_p}}}\xspace}  
\newcommand{\bimpact}{\ensuremath{b}\xspace} 	
\newcommand{\rprstar}{\ensuremath{R_{\mathrm{p}}/R_*}\xspace} 	
\newcommand{\ted}{\ensuremath{ED}\xspace} 	
\newcommand{\lp}{\ensuremath{L_{\mathrm{p}}}\xspace} 	
\newcommand{\lplstar}{\ensuremath{\frac{L_{\mathrm{p}}}{L_*}}\xspace} 	
\newcommand{\gcm}{\ensuremath{\rm{g\,cm^{-3}}}\xspace} 
\newcommand{\gravunits}{\ensuremath{\rm{cm^{2}\,g^{-1}\,s^{-2}}}\xspace} 		
\newcommand{\msec}{\ensuremath{\rm{m\,s^{-1}}}\xspace} 	

\newcommand{\wmf}{\ensuremath{\rm{WMF}}\xspace} 	
\newcommand{\water}{\ensuremath{\rm{H_{2}O}}\xspace} 	
\newcommand{\logwmf}{\ensuremath{\rm{log(WMF)}}\xspace} 	

\newcommand{\mocean}{\ensuremath{\it{M}_{\rm{ocean}}}\xspace} 	
\newcommand{\mwater}{\ensuremath{\it{M}_{\rm{\water}}}\xspace} 	
\newcommand{\massf}{\ensuremath{\it{M}_{\rm{f}}}\xspace} 	

\newcommand{\vrelvesc}{\ensuremath{v_{rel}/v_{esc}}\xspace} 	
\newcommand{\vimpvesc}{\ensuremath{v_{imp}/v_{esc}}\xspace} 	
\newcommand{\ecc}{\ensuremath{e}\xspace} 	
\newcommand{\inc}{\ensuremath{i}\xspace} 	
\newcommand{\bimp}{\ensuremath{b}\xspace} 		

\newcommand{\mimpmtar}{\ensuremath{m_{imp}/m_{tar}}\xspace} 	

\newcommand{\rtar}{\ensuremath{r_{tar}}\xspace} 	
\newcommand{\rimp}{\ensuremath{r_{imp}}\xspace} 	

\newcommand{\semimajf}{\ensuremath{\it{a}_\rm{f}}\xspace} 	
\newcommand{\eccf}{\ensuremath{\it{e}_f}\xspace} 	
\newcommand{\incf}{\ensuremath{\it{i}_f}\xspace} 	
\newcommand{\semimajin}{\ensuremath{\it{a}_{in}}\xspace} 	
      



